Spatial-Temporal Hypergraph Self-Supervised Learning for Crime Prediction

Crime has become a major concern in many cities, which calls for the rising demand for timely predicting citywide crime occurrence. Accurate crime prediction results are vital for the beforehand decision-making of government to alleviate the increasing concern about the public safety. While many efforts have been devoted to proposing various spatial-temporal forecasting techniques to explore dependence across locations and time periods, most of them follow a supervised learning manner, which limits their spatial-temporal representation ability on sparse crime data. Inspired by the recent success in self-supervised learning, this work proposes a Spatial-Temporal Hypergraph Self-Supervised Learning framework (ST-HSL) to tackle the label scarcity issue in crime prediction. Specifically, we propose the cross-region hypergraph structure learning to encode region-wise crime dependency under the entire urban space. Furthermore, we design the dual-stage self-supervised learning paradigm, to not only jointly capture local- and global-level spatial-temporal crime patterns, but also supplement the sparse crime representation by augmenting region self-discrimination. We perform extensive experiments on two real-life crime datasets. Evaluation results show that our ST-HSL significantly outperforms state-of-the-art baselines. Further analysis provides insights into the superiority of our ST-HSL method in the representation of spatial-temporal crime patterns. The implementation code is available at https://github.com/LZH-YS1998/STHSL.

==> coverletter.tex <==


\section*{Response to Reviewers}

We really appreciate the constructive comments of all reviewers, and have carefully addressed them in our revision. The main revisions include clarifications in relevant subsections, additional experiments for further justification of our method, more detailed discussions on the experimental results, more references suggested by the reviewers and etc. The updated parts in our revision are highlighted with red color.

\subsection{Response to Reviewer \#1}

We would like to thank the reviewer for their careful reading and helpful comments. We have revised the manuscript to address the questions raised by the reviewer.

\textbf{Comment 1}: Explanation of auxiliary supervision labels in self-supervised learning paradigm.\\\vspace{-0.15in}

\textbf{Response}: Self-supervised methods rely on two types of training signals for model inference, i.e., original labels and auxiliary supervision signals. As the reviewer says, pre-training can be considered as a type of self-supervised learning strategy which trains neural networks with specific unsupervised objectives, so as to address the limitation of random parameter initialization. In this work, our framework is designed based on another type of self-supervised learning paradigm which integrates the generative and contrastive self-supervised objectives as auxiliary training signals. In addition to $X_{T+1}$ ground truth of crime occurrence, our method supplements the supervised prediction on sparse crimes with dual-stage auxiliary self-supervised tasks (local-global region contrastive learning and hypergraph infomax network), to enhance the representation of crime patterns. To address the reviewer's comment, we add more explanation in the related work section (Section V.D) to clarify this point.\\\vspace{-0.1in}

\textbf{Comment 2}: Explanation of STSHN's performance.\\\vspace{-0.15in}

\textbf{Response}: From the description and released implementation code, STSHN method conducts the prediction on regions with the crime density degrees larger than 0.2 and ignores the regions with sparse crime labels. For more comprehensive evaluations, we perform the crime prediction on all regions. With the crime forecasting on all regions (including more sparse regions), STSHN performs worse than prediction on denser regions. With our designed hypergraph-enhanced contrastive learning paradigms, our method outperforms STSHN baseline in all cases.\\\vspace{-0.1in}

\textbf{Comment 3}: Model efficiency study.\\\vspace{-0.15in}

\textbf{Response}: While our method ST-HSL requires larger computational cost compared with the baseline STtrans, ST-HSL significantly improves the crime prediction accuracy as compared to STtrans (as shown in Table III for overall performance comparison). In addition, we further conduct experiments to evaluate the model robustness of our ST-HSL method and STtrans on regions with different sparsity degrees. Particularly, the results (measured by MAE) are as follows: i) NYC data: for our ST-HSL method, (0,0.25]-0.7822; (0.25,0.5]-0.6410; (0.5,0.75]-0.7630; (0.75,1]-1.2359; for baseline STtrans, (0,0.25]-0.9544; (0.25,0.5]-0.7865; (0.5,0.75]-0.7870; (0.75,1]-1.2808. ii) Chicago data: for our ST-HSL method, (0,0.25]-0.6485; (0.25,0.5]-0.5436; (0.5,0.75]-0.7292; (0.75,1]-1.3399.; for baseline STtrans, (0,0.25]-0.9300; (0.25,0.5]-0.7555; (0.5,0.75]-0.7642; (0.75,1]-1.3435. Note that low MAE value indicates better performance. We can observe that ST-HSL consistently significantly outperforms STtrans in all cases, which further demonstrates the superiority of our ST-HSL method compared with STtrans in offering better crime forecasting accuracy. The computational cost of our approach stem from two key perspectives: i) hypergraph-enhanced global region-wise dependency modeling; ii) dual-stage self-supervised learning tasks for data augmentation. Additionally, our new method achieves better model efficiency compared with several strong baselines. To address this comment, we add more discussion in Section IV.G.\\\vspace{-0.1in}

\textbf{Comment 4}: Explanation of anchor.\\\vspace{-0.15in}

\textbf{Response}: The anchor embedding is the learned representation of the target region. Based on the self-discrimination design, we treat the encoded embeddings from the local relation modeling and the global cross-region dependency modeling as positive training pairs, and embeddings of different regions are regarded as negative samples.\\\vspace{-0.1in}

\textbf{Comment 5}: Comparison with suggested baselines.\\\vspace{-0.15in}

\textbf{Response}: To address reviewer’s comment, we compare our method with the suggested baselines (i.e., GWN, AGCRN, MTGNN, EnhanceNet). The overall performance (measured by MAPE) across different types of crimes is: for NYC data, STHSL: 0.4889, GWN: 0.5411, AGCRN: 0.5423, MTGNN: 0.5465, EnhanceNet: 0.5335; for Chicago dataset, STHSL: 0.4784, GWN: 0.5189, AGCRN: 0.5190, MTGNN: 0.5178, EnhanceNet: 0.5028. Given the results, our STHSL outperforms all baselines on different datasets, which further demonstrates the effectiveness of our spatial-temporal hypergraph-enhanced self-supervised learning framework. New evaluation results of suggested baselines are updated in Table III for performance comparison on both NYC and Chicago datasets in terms of MAE and MAPE. In addition, the description of new added baselines are updated in Section IV. A 3) Baselines for comparison.\\\vspace{-0.1in}

\textbf{Comment 6}: Further explanation of how challenges are addressed by the proposed techniques.\\\vspace{-0.15in}

\textbf{Response}: To address the sparse supervision signal challenge, our designed hypergraph-enhanced dependency modeling component can capture the holistic crime occurrence patterns and preserve the global spatial context by performing the knowledge transfer across the entire urban space. To address the skewed crime data distribution challenge under the global relation learning, the developed dual-stage self-supervised learning framework, which integrates hypergraph contrastive learning and hypergraph infomax network, endows our learning of crime patterns with auxiliary self-supervision signals under sparse crime data.\\\vspace{-0.1in}

\subsection{Response to Reviewer \#2}

\textbf{Comment 1}: Explanation of input tensor size.\\\vspace{-0.15in}

\textbf{Response}: In our temporal convolutional encoder, with the consideration of region geographical locations, the input tensor dimension should be $\mathbf{E}_t \in \mathbb{R}^{I\times J\times C \times d}$ in Equation (2), where $I$ and $J$ represents the number of regions respectively corresponding to the row and column dimension in the spatial region map in a city. In the rest of solution section, the input dimension of data tensor over the region dimension can be represented as $R$. To address this comment, we add more explanations in Section III.B 1). \\\vspace{-0.1in}

\textbf{Comment 2}: Explanation of Figure 2. \\\vspace{-0.15in}

\textbf{Response}: In Figure 2, we show the skewed distribution of crime occurrence with different types at different regions in New York City on September 2015. The y-axis represents the number of crime cases reported from the time period, and x-axis denotes the region index. For better presentation for the long-tail crime distribution, we sort the region index (x-axis) in terms of the number of crime cases. Therefore, each bar in those figures represent the number of happened crimes with a certain crime category at a specific region. The explanation has been added in the paragraph of Section I.\\\vspace{-0.1in}

\textbf{Comment 3}: Explanation of dealing with the data skewed distribution challenge with our hypergraph structure learning.\\\vspace{-0.15in}

\textbf{Response}: To address the crime skewed distribution challenge, our hypergraph relation learning framework endows our cross-region relation modeling with the capability of global context awareness. By effectively encoding the relevance between different regions and latent hyperedge representations, regions with similar crime distributions across the entire city can be correlated for knowledge transfer with the injecting global urban context. By doing so, we can alleviate the skewed distribution issue. The explanation of dealing with skewed data distribution has been added in the first and third paragraphs of Section III.\\\vspace{-0.1in}

\textbf{Comment 4}: Explanation of hyperedge settings.\\\vspace{-0.15in}

\textbf{Response}: The choice of $H$ depends on the city scale. The number of hyperedges is selected from the range {32, 64, 128, 256}. The best prediction performance is achieved on both NYC and Chicago with $H=128$, since NYC and Chicago are both large-scale cities in US. After collecting more available crime datasets, we will evaluate our algorithm on small-scale cities. The explanation of hyperedge settings has been updated in Section IV.A 4). \\\vspace{-0.1in}

\textbf{Comment 5}: Discuss the suggested related work.\\\vspace{-0.15in}

\textbf{Response}: The suggested work [1] aims to capture the dynamics and heterogeneity over spatial-temporal graph. Different from it, we proposed a spatial-temporal self-supervised learning framework with hypergraph structure learning architecture to capture dynamic crime patterns under data scarcity. \\\vspace{-0.1in}

[1] Learning Dynamics and Heterogeneity of Spatial-Temporal Graph Data for Traffic Forecasting, TKDE 2021.

\subsection{Response to Reviewer \#3}

\textbf{Comment 1}: Performance comparison with a suggested variant in the model ablation study.\\\vspace{-0.15in}

\textbf{Response}: To address reviewer’s comment, we compare our STHSL with the variant (Fusion w/o ConL)-by directly fusing the encoded local and global embeddings without the incorporation of contrastive objective. The overall evaluation results across types (measured by MAPE) are: for NYC dataset, ST-HSL: 0.4889, Fusion w/o ConL: 0.5364; for Chicago dataset, ST-HSL: 0.4784, Fusion w/o ConL: 0.5122. The effectiveness of our local-global contrastive learning can be validated with the superior performance. Contrastive learning paradigm in our ST-HSL framework allows the model to explore useful information from the data itself, which is helpful to generate more robust feature representation.. To address this comment, new results are added in the section of model ablation study (Section IV.C 2)).\\\vspace{-0.1in}

\textbf{Comment 2}: Explanation of using global view representation for prediction. \\\vspace{-0.15in}

\textbf{Response}: Thanks for the valuable feedback. We conduct experiment to further evaluate the suggested embedding fusion method with the consideration of both local and global views. Specifically, we generate a corresponding model variant Fusion-LG in the model ablation study. From the updated evaluation results in Table IV, we can observe that the better performance can be achieved by using the global view embedding for prediction (ST-HSL) as compared to using both local and global embeddings (Fusion-LG). In the prediction layer, we can consider the embedding fusion layer as a flexible readout operation by taking either local-view or global-view latent representations for making prediction. \\\vspace{-0.1in}

\textbf{Comment 3}: The sum over all dimensions is used in Eq.9.\\\vspace{-0.15in}

\textbf{Response}: Thanks for pointing out this typo in Eq 9. We have fixed it by adding d' as the dimension index. We differentiate the weights for transformation of each latent dimension. In Eq 9, The weight parameters $\textbf{W}_{d}\in\mathbb{R}^{d\times d}$ is applied to latent dimensions with different weights. \\\vspace{-0.1in}

\textbf{Comment 4}: Explanation of temporal convolutional network as the temporal encoder. \\\vspace{-0.15in}

\textbf{Response}: Since our framework is model-agnostic for temporal encoder, we only perform 1D convolutions over time dimension for temporal dependency modeling. Our STHSL is general and flexible to integrate with complex TCNs.
